Batch weight for domain adaptation with mass shift

Unsupervised domain transfer is the task of transferring or translating samples from a source distribution to a different target distribution. Current solutions unsupervised domain transfer often operate on data on which the modes of the distribution are well-matched, for instance have the same frequencies of classes between source and target distributions. However, these models do not perform well when the modes are not well-matched, as would be the case when samples are drawn independently from two different, but related, domains. This mode imbalance is problematic as generative adversarial networks (GANs), a successful approach in this setting, are sensitive to mode frequency, which results in a mismatch of semantics between source samples and generated samples of the target distribution. We propose a principled method of re-weighting training samples to correct for such mass shift between the transferred distributions, which we call batch-weight. We also provide rigorous probabilistic setting for domain transfer and new simplified objective for training transfer networks, an alternative to complex, multi-component loss functions used in the current state-of-the art image-to-image translation models. The new objective stems from the discrimination of joint distributions and enforces cycle-consistency in an abstract, high-level, rather than pixel-wise, sense. Lastly, we experimentally show the effectiveness of the proposed methods in several image-to-image translation tasks.

==> table-0.tex <==
\begin{table}*
    \centering
    \begin{tabular}{cc}
         model & multimodal & unpaired & loss components \\
         \hrule\hrule
         CycleGAN \citep{cycle-gan} & \xmark & \checkmark & 2 \\
         BiCycleGAN \citep{bicyclegan} & \checkmark & \xmark & 5
         DRIT \citep{drit} & \checkmark & \checkmark & 6 \\
         MUNIT \citep{munit} & \checkmark & \checkmark & 5 \\
         \hrule
         proposed & \checkmark & \checkmark & 1
    \end{tabular}
    \caption{Overview of image-to-image transfer models.}
    \label{t:overview}
\end{table}*
